Mitigating Advanced Adversarial Attacks with More Advanced Gradient Obfuscation Techniques

Deep Neural Networks (DNNs) are well-known to be vulnerable to Adversarial Examples (AEs). A large amount of efforts have been spent to launch and heat the arms race between the attackers and defenders. Recently, advanced gradient-based attack techniques were proposed (e.g., BPDA and EOT), which have defeated a considerable number of existing defense methods. Up to today, there are still no satisfactory solutions that can effectively and efficiently defend against those attacks. In this paper, we make a steady step towards mitigating those advanced gradient-based attacks with two major contributions. First, we perform an in-depth analysis about the root causes of those attacks, and propose four properties that can break the fundamental assumptions of those attacks. Second, we identify a set of operations that can meet those properties. By integrating these operations, we design two preprocessing functions that can invalidate these powerful attacks. Extensive evaluations indicate that our solutions can effectively mitigate all existing standard and advanced attack techniques, and beat 11 state-of-the-art defense solutions published in top-tier conferences over the past 2 years. The defender can employ our solutions to constrain the attack success rate below 7% for the strongest attacks even the adversary has spent dozens of GPU hours.

==> sections/04-methodology-v1.tex <==
\section{Methodology Insights and Overview}
\label{sec:overview}

Our proposed defense solution is a preprocessing function $g(x)$, which can defeat the advanced attacks with the threat model in Section \ref{sec:threat-model} and satisfy the requirements in Section \ref{sec:def-req}. In this section, we analyze these attacks and identify the design philosophy of our methodology. We give specific examples of qualified functions in the next section. 

\subsection{Mitigation of Gradient Approximation Attacks}
\label{sec:method-bpda}

\noindent{\textbf{Attack analysis.}} As mentioned in Section~\ref{sec:devep-hist}, for shattered gradient based defense solutions, an non-differentiable operation ($g(\cdot)$) is integrated with the target model $f(\cdot)$ to preprocess the input samples, then the model inference process becomes $y=f(g(x))$. This can increase the difficulty of calculating gradients directly, since $g(x)$ is non-differentiable. Thus AE generation becomes infeasible. 

%$\bigtriangledown _{x}f(g(x))| _{x = \hat{x}} = \bigtriangledown _{x} f(x)| _{x = g(\hat{x})}\bigtriangledown _{x} g(x) | _{x = \hat{x}}$

To solve this problem, BPDA attack technique was proposed~\cite{athalye2018obfuscated}. The key assumption is that the preprocessing function $g$ should maintain the property $g(x)\approx x$ in order to preserve the functionality of the target model $f(\cdot)$. 
\qiuhan{To defeat such defense, BPDA attack was proposed~\cite{athalye2018obfuscated}. with a key assumption that the preprocessing function $g(\cdot)$ maintains the property $g(x)\approx x$ in order to preserve the functionality of the target model $f(\cdot)$. }
This assumption is held for all existing shattered gradient based solutions. Then the adversary can use $g(x)$ on the forward pass and replace it with $x$ on the backward pass when calculating the gradients. The derivative of the preprocessing function will be approximated as the derivative of the identity function, which is 1\qiuhan{what is 1?}. The gradient calculation process is described in Equation \ref{eq:bpda1}. 

\begin{subequations}
\label{eq:bpda1}
  \begin{align}
\bigtriangledown _{x}f(g(x))| _{x = \hat{x}} & = \bigtriangledown _{x} f(x)| _{x = g(\hat{x})} \times \bigtriangledown _{x} g(x) | _{x = \hat{x}} \\
& \approx \bigtriangledown _{x} f(x)| _{x = g(\hat{x})} \times \bigtriangledown _{x} x | _{x = \hat{x}} \\
& = \bigtriangledown _{x} f(x)| _{x = g(\hat{x})}
  \end{align}
\end{subequations}

\noindent{\textbf{Attack mitigation.}}
We identify several necessary properties %Yi -- sufficient or necessary
of the preprocessing function $g(x)$ in order to mitigate BPDA attack. First, this function must preserve the functionality of the target model, without affecting the prediction results of normal samples. This gives the first property for our solution:

\REQ{1}{$g(x)$ cannot affect the prediction results: $f(g(x)) = f(x)$}.

The BPDA attack depends on the condition that $g(x) \approx x$. To invalidate such attack, we need to design a preprocessing function that can break this assumption. This leads to the second property as below. Note that Properties \#1 and \#2 are not contradictory. It is possible (although challenging) to identify such preprocessing functions that can satisfy both properties. We will show detailed examples in Section \ref{sec:analyze}

\REQ{2}{$g(x)$ cannot be approximated as $x$: $g(x) \not\approx x$}

We should also consider more adaptive attacks. Even the adversary cannot use $x$ to replace $g(x)$ for gradient calculation with properties \#1 and \#2, it is still possible that he might discover an alternative differentiable function \qiuhan{differentiable function is not correct} to approximate $g(x)$. To eliminate such possibility, we can obfuscate the function with randomization. This is the third property: 

\REQ{3}{$g(x)$ cannot be approximated as a differentiable function $g'(x)$.}\qiuhan{REQ3 is not correct. g(x) is random but is differentiable.}

\subsection{Mitigation of Gradient Expectation Attacks}
 
\noindent{\textbf{Attack analysis.}} 
Another popular preprocessing operation is to randomize the gradient of the model in real-time without affecting the prediction results. To evade such defense strategy, EoT was adopted as an attack strategy~\cite{athalye2018obfuscated}, which statistically computes the gradients over the expected transformation to the input $x$. Formally, for a preprocessing function $g(x)$ that randomly transforms $x$ from a distribution of transformations $T$, EoT optimizes the expectation over the transformation with respect to the input by $\mathbb{E} _{t\sim T}f(g(x))$, as shown in Eq. \ref{eq:eot1}. The adversary can always get a proper expectation with samples at each gradient descent step. 

\begin{equation}\label{eq:eot1}
	\bigtriangledown_{x}  \mathbb{E} _{t\sim T}f(g(x)) = \mathbb{E} _{t\sim T} \bigtriangledown_{x} f(g(x))
\end{equation}


\noindent{\textbf{Attack mitigation.}}
EoT needs to calculate the gradient of $f(g(x))$ in Eq. \ref{eq:eot1} to calculate the expectation over the transformation. It needs the requirement that $g(x)$\qiuhan{$t(x)$ to represent the non-differentiable function} is differentiable. This gives us the last property for our preprocessing strategy to mitigate EoT attack: 

\REQ{4}{$g(x)$ is non-differentiable.} 

\subsection{Put Everything Together}
\label{sec:method-bpda+eot}

In reality it is difficult to discover a single operation that can meet all the four properties. To simplify this problem, we can concatenate two operations: $g = g_1 \circ g_2$. Operation $g_1$ focuses on the gradient approximation attack, with properties \#2 and \#3. Operation $g_2$ focuses on the gradient expectation attack, with property \#4. Both two operations have property \#1. The integration of them can mitigate advanced attacks (BPDA, EoT or their combination), as well as simple attacks (e.g., FGSM, LBFGS, C\&W). We present the analysis below. 
 
\noindent{\textbf{Mitigating Simple Attacks.}} 
Operation $g_1$ can lead to stochastic gradients caused by the randomization factor. Operation $g_2$ can give shattered gradients. As the result, Function $g$ enjoys both of the two obfuscation features, and can defeat simple attacks as other preprocessing-based solutions. 

\noindent{\textbf{Mitigating Advanced Attacks.}}
Due to the non-differentiable $g_2$, it is impossible to employ EoT only to compromise the function $g(x)$. The adversary can ignore the existence of $g_2$ and use EoT to generate perturbations only from $f(x)$ and $g_1(x)$. Such AEs cannot fool the model expected by the adversary, as the operation $g_2(x)$ can invalidate the perturbation at the inference stage. Empirical evaluations can be found in Section \ref{sec:eval}.

Due to properties \#2 and \#3 of $g_1$, the BPDA technique cannot get the correct gradients and optimal perturbation. The integration of BPDA and EoT techniques can remove the obstruction from property \#3. However, property \#2 can still hinder the adversary from generating effective AEs. We can see this is the essential property to mitigate advanced attacks, which existing solutions do not have.

==> sections/06-setup.tex <==






==> tables/table-hybrid-approch.tex <==
\iffalse

\begin {table}[t]\centering
\begin{tabular}{ c |c  } \hline
\textbf{Monitoring use case}  & \textbf{Metric access approach} \\  \hline \hline
Continuous UE connectivity    & \textit{Push} \\ 
Hotspot detection             & \textit{Push} \\ 
Real-time troubleshooting     & \textit{Push} \\ 
Critical event                & \textit{Push with real-time} \\ 
System-level metrics          & \textit{Pull} \\ 
Infrastructure-level metrics  & \textit{Pull} \\ 
IoT                           & \textit{Push and Pull}   \\   \hline
\end{tabular}\caption{A requirement of the hybrid monitoring approach in 5G}
\label{table:monitoring-approach}
\end {table}
\fi
